Multimodal Privacy-preserving Mood Prediction from Mobile Data: A Preliminary Study

Mental health conditions remain under-diagnosed even in countries with common access to advanced medical care. The ability to accurately and efficiently predict mood from easily collectible data has several important implications towards the early detection and intervention of mental health disorders. One promising data source to help monitor human behavior is from daily smartphone usage. However, care must be taken to summarize behaviors without identifying the user through personal (e.g., personally identifiable information) or protected attributes (e.g., race, gender). In this paper, we study behavioral markers or daily mood using a recent dataset of mobile behaviors from high-risk adolescent populations. Using computational models, we find that multimodal modeling of both text and app usage features is highly predictive of daily mood over each modality alone. Furthermore, we evaluate approaches that reliably obfuscate user identity while remaining predictive of daily mood. By combining multimodal representations with privacy-preserving learning, we are able to push forward the performance-privacy frontier as compared to unimodal approaches.

==> preprint2020_Mobile Data/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{eq~(\ref{#1})}
% Reference to an equation, upper case
\def\Eqref#1{Eq~(\ref{#1})}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} 

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\usepackage{hyperref}

\usepackage{booktabs}       %
\usepackage{amsfonts}       %
\usepackage{nicefrac}       %
\usepackage{microtype}      %
\usepackage{subcaption}

\usepackage{enumitem}
\setlist{nolistsep}
\setlist[itemize]{noitemsep, topsep=0pt}

\usepackage{times}

\usepackage{graphicx} %
\usepackage{color}

\usepackage{array}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{xspace}
\usepackage{fancyhdr}
\usepackage{comment}

\newcommand{\mycaptionof}[2]{\captionof{#1}{#2}}

\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}}

\newcommand{\noaistats}[1]{}  %

\definecolor{darkgreen}{rgb}{0,0.4,0.0}
\definecolor{darkblue}{rgb}{0,0.1,0.3}
\definecolor{darkred}{rgb}{0.7,0.0,0.0}

\newcommand{\lbs}{\ensuremath{B}}      %
\newcommand{\all}{\infty}
\newcommand{\lepochs}{\ensuremath{E}}  %
\newcommand{\clientfrac}{\ensuremath{C}}    %
\newcommand{\tnn}{2NN\xspace} %
\newcommand{\xx}{\hspace{-0.01in}\ensuremath{\times}}
\newcommand{\loss}{\ell}
\newcommand{\SUB}[1]{\ENSURE \hspace{-0.15in} \textbf{#1}}
\newcommand{\algfont}[1]{\texttt{#1}}

\renewcommand{\algorithmicensure}{}

\newcommand{\T}{\rule{0pt}{2.2ex}}
\newcommand{\targetTNN}{97\%\xspace}
\newcommand{\targetCNN}{99\%\xspace}
\newcommand{\targetLSTM}{54\%\xspace}
\newcommand{\nc}{K}
\newcommand{\pp}{\mathcal{P}}


\newlength{\pw}


\newcommand{\BO}{\mathcal{O}}
\newcommand{\qqand}{\qquad \text{and} \qquad}
\newcommand{\qqwhere}{\qquad \text{where} \qquad}
\newcommand{\qqwith}{\qquad \text{with} \qquad}
\newcommand{\grad}{\triangledown}
\newcommand{\h}{\frac{1}{2}}


==> preprint2020_Mobile Data/tables/MLP_hyperparameters_apps.tex <==
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{MLP parameter configuration (Apps).}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l | c}
\Xhline{3\arrayrulewidth}
Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
hidden dim 1 & 128 \\
hidden dim 2 & 128, 64 \\
dropout rate & 0, 0.2, 0.5 \\
learning rate & 0.001 \\
batch size & 100 \\
epochs & 200 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{mlp_params_apps}
\end{table*}

==> preprint2020_Mobile Data/tables/MLP_hyperparameters_bow.tex <==
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{MLP parameter configuration (Combined, BoW).}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l | c}
\Xhline{3\arrayrulewidth}
Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
hidden dim 1 & 1024, 512 \\
hidden dim 2 & 128, 64 \\
dropout rate & 0, 0.2, 0.5 \\
learning rate & 0.001 \\
batch size & 100 \\
epochs & 200 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{mlp_params_bow}
\end{table*}

==> preprint2020_Mobile Data/tables/SAL_hyperparameters.tex <==
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{\names\ parameter configuration.}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l | c}
\Xhline{3\arrayrulewidth}
Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
$\lambda$ & 0.1, 1, 2, 3, 5, 10 \\
$\sigma$ & 1, 5, 10, 25, 50, 100 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{sal_params}
\end{table*}

==> preprint2020_Mobile Data/tables/SVM_hyperparameters.tex <==
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{SVM parameter configuration. \\
*Integer kernel values denote the degree of a polynomial kernel.}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l | c }
\Xhline{3\arrayrulewidth}
Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
C & 0.1, 0.5, 1, 2, 3, 5, 10 \\
Kernel* & RBF, 2, 3, 5, 10 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{svm_params}
\end{table*}

==> preprint2020_Mobile Data/tables/hyperparameters.tex <==
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{Model parameter configurations. \\
*Integer kernel values denote the degree of a polynomial kernel.}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l | c | c }
\Xhline{3\arrayrulewidth}
Model & Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
\multirow{2}{*}{SVM}
& C & 0.1, 0.5, 1, 2, 3, 5, 10 \\
& Kernel* & RBF, 2, 3, 5, 10 \\
\Xhline{0.5\arrayrulewidth}
\multirow{6}{*}{MLP}
& hidden dim 1 & 1024, 512, 128 \\
& hidden dim 2 & 128, 64 \\
& dropout rate & 0, 0.2, 0.5 \\
& learning rate & 0.001 \\
& batch size & 100 \\
& epochs & 200 \\
\Xhline{0.5\arrayrulewidth}
\multirow{2}{*}{\names}
& $\lambda$ & 0.1, 1, 2, 3, 5, 10 \\
& $\sigma$ & 1, 5, 10, 25, 50, 100 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{params}
\end{table*}

==> preprint2020_Mobile Data/tables/modalities_comparison.tex <==
\definecolor{gg}{RGB}{15,125,15}
\definecolor{rr}{RGB}{190,45,45}

\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\vspace{-4mm}
\centering
\caption{Comparison of mood prediction performance across different modalities. Best results in \textbf{bold}. For both accuracy and F1 score, models trained on both text and apps features outperform models trained using individual modalities. $\star$ and $\diamond$ denote that the difference between multimodal and unimodal (Text and Apps respectively) is statistically significant (p-value $<< 0.05$).}
\setlength\tabcolsep{5.0pt}
\begin{tabular}{l || c c c c | c c c c }
\Xhline{3\arrayrulewidth}
& \multicolumn{4}{c|}{{F1 score}} & \multicolumn{4}{c}{{Accuracy}} \\
Modalities & \textsc{Baseline} & \textsc{SVM} & \textsc{MLP} & \names &  \textsc{Baseline} & \textsc{SVM} & \textsc{MLP} & \names \\
\Xhline{0.5\arrayrulewidth}
Text + Apps &  $19.07$ & $\textbf{62.08}^{\diamond}$ & $\textbf{58.38}^{\star\diamond}$ & $\textbf{52.90}$ & $40.18$ & $\textbf{66.59}^{\diamond}$ & $\textbf{62.93}^{\star\diamond}$ & $\textbf{56.76}$ \\
Text & $19.07$ & $61.15 $ & $56.27$ & $52.63$ & $40.18$ & $65.83$ & $60.61$ & $56.08$ \\
Apps & $19.07$ & $58.65$ & $52.29$ & $51.32$ & $40.18$ & $62.65$ & $55.26$ & $55.68$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{modalities_comparison}
\end{table*}

==> preprint2020_Mobile Data/tables/model_comparison.tex <==
\definecolor{gg}{RGB}{15,125,15}
\definecolor{rr}{RGB}{190,45,45}

\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{mood prediction}
\setlength\tabcolsep{5.0pt}
\begin{tabular}{l || c | c c c | c c c | c c c}
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{} & \multirow{2}{*}{Baseline} & \multicolumn{3}{c|}{{Text+Apps}} & \multicolumn{3}{c|}{{Text}} & \multicolumn{3}{c}{{Apps}} \\
& & \textsc{SVM} & \textsc{MLP} & \names & \textsc{SVM} & \textsc{MLP} & \names & \textsc{SVM} & \textsc{MLP} & \names \\
\Xhline{0.5\arrayrulewidth}
accuracy & $40.18$ & $66.59$ & $62.93$ & $55.49$ & $65.83$ & $60.61$ & $53.53$ & $62.65$ & $55.26$ & $54.20$ \\
average F1 & $19.07$ & $62.08$ & $58.38$ & $50.43$ & $61.15$ & $56.27$ & $47.98$ & $58.65$ & $52.29$ & $49.40$ \\
%balanced acc. & $33.33$ & $62.62$ & $61.34$ & $55.44$ & $61.43$ & $59.57$ & $54.16$ & $62.08$ & $56.95$ & $52.83$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{model_comparision}
\end{table*}

==> preprint2020_Mobile Data/tables/privacy.tex <==
\definecolor{gg}{RGB}{15,125,15}
\definecolor{rr}{RGB}{190,45,45}

\begin{table*}[t!]
\vspace{-4mm}
\begin{minipage}{.45\linewidth}
\fontsize{9}{11}\selectfont
\caption{\textbf{Left:} We evaluate privacy in predicting user identity from representations learned by \textsc{MLP} and \names\ (\textbf{lower} accuracy is better), and find that \names\ effectively obfuscates user identity. \textbf{Right:} Tradeoff between performance (mood prediction F1 score, \textbf{higher} is better) and privacy (identity prediction accuracy, \textbf{lower} is better) \names\ provides a tunable parameter $\sigma$ which allows us to plot a range of (performance, privacy) points. Furthermore, using a multimodal model on text and app features pushes the Pareto front to obtain better performance and privacy at the same time.}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l || c c c }
\Xhline{3\arrayrulewidth}
& Text + Apps & Text & Apps \\
\Xhline{0.5\arrayrulewidth}
Raw features & $95.70$ & $92.65$ & $91.82$ \\ 
\textsc{MLP} & $79.04$ & $76.41$ & $85.94$ \\ 
\names & $\textbf{36.65}$ & $\textbf{38.38}$ & $\textbf{36.72}$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{privacy}
%
\end{minipage}
\hspace{4mm}
\vspace{-4mm}
\begin{minipage}{.55\linewidth}
\centering
\includegraphics[width=\textwidth]{images/tradeoff.png}
\end{minipage}

\vspace{-2mm}
\end{table*}

==> preprint2020_Mobile Data/tables/pvalue_compare_modalities.tex <==
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{Comparing multimodal to single modalities}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l l || c c | c c }
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{} & \multirow{2}{*}{} & \multicolumn{2}{c|}{{Combined $\minus$ Text}} & \multicolumn{2}{c}{{Combined $\minus$ Apps}}  \\
& & $\Delta$ & p-value & $\Delta$ & p-value \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SVM}
& \multirow{1}{*}{accuracy} & $0.75$ & $0.2537$ & $3.93$ & $0.0038$ \\
& \multirow{1}{*}{balanced acc.} & $1.19$ & $0.1206$ & $0.54$ & $0.6768$ \\
& \multirow{1}{*}{average F1} & $0.92$ & $0.1664$ & $3.42$ & $0.0083$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{MLP}
& \multirow{1}{*}{accuracy} & $2.33$ & $0.0095$ & $7.67$ & $0.0025$ \\
& \multirow{1}{*}{balanced acc.} & $1.77$ & $0.0109$ & $4.39$ & $0.0035$ \\
& \multirow{1}{*}{average F1} & $2.11$ & $0.0183$ & $6.09$ & $0.0025$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SAL}
& \multirow{1}{*}{accuracy} & $1.96$ & $0.0463$ & $0.78$ & $0.3994$ \\
& \multirow{1}{*}{balanced acc.} & $1.28$ & $0.1931$ & $1.76$ & $0.2223$ \\
& \multirow{1}{*}{average F1} & $2.45$ & $0.234$ & $-0.10$ & $0.6006$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{pvalue_compare_modalities}
\end{table*}

\iffalse
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{p-value compared modalities (maybe include? really only MLP seems easy to talk about since it's clearly that Combined > BoW > App since they're all statistically significant. not really the case for svm though and def not for SAL)}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l l || c c | c c | c c }
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{} & \multirow{2}{*}{} & \multicolumn{2}{c|}{{Combined $\minus$ BoW}} & \multicolumn{2}{c|}{{Combined $\minus$ Apps}} & \multicolumn{2}{c}{{BoW $\minus$ Apps}} \\
& & $\Delta$ & p-value & $\Delta$ & p-value & $\Delta$ & p-value\\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SVM}
& \multirow{1}{*}{accuracy} & $0.75$ & $0.2537$ & $3.93$ & $0.0038$ & $3.18$ & $0.0183$ \\
& \multirow{1}{*}{balanced acc.} & $1.19$ & $0.1206$ & $0.54$ & $0.6768$ & $-0.65$ & $0.6394$ \\
& \multirow{1}{*}{average F1} & $0.92$ & $0.1664$ & $3.42$ & $0.0083$ & $2.50$ & $0.1013$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{MLP}
& \multirow{1}{*}{accuracy} & $2.33$ & $0.0095$ & $7.67$ & $0.0025$ & $5.35$ & $0.0063$ \\
& \multirow{1}{*}{balanced acc.} & $1.77$ & $0.0109$ & $4.39$ & $0.0035$ & $2.62$ & $0.0463$ \\
& \multirow{1}{*}{average F1} & $2.11$ & $0.0183$ & $6.09$ & $0.0025$ & $3.98$ & $0.0142$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SAL}
& \multirow{1}{*}{accuracy} & $1.96$ & $0.0463$ & $0.78$ & $0.3994$ & $-1.18$ & $0.7462$ \\
& \multirow{1}{*}{balanced acc.} & $1.28$ & $0.1931$ & $1.76$ & $0.2223$ & $0.49$ & $0.3994$ \\
& \multirow{1}{*}{average F1} & $2.45$ & $0.234$ & $-0.10$ & $0.6006$ & $-2.54$ & $0.9156$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{pvalue_compare_modalities}
\end{table*}
\fi

==> preprint2020_Mobile Data/tables/pvalue_compare_to_baseline.tex <==

\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{p-value compared to baseline (seems pretty messy. don't want to include, will just say p-value is significant across all models, features, and metrics)}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l l || c c | c c | c c }
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{} & \multirow{2}{*}{} & \multicolumn{2}{c|}{{Combined}} & \multicolumn{2}{c|}{{Text}} & \multicolumn{2}{c}{{Apps}} \\
& & $\Delta$ & p-value & $\Delta$ & p-value & $\Delta$ & p-value\\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SVM}
 & \multirow{1}{*}{accuracy} & $26.41$ & $<0.005$ & $25.65$ & $<0.005$  & $22.47$ & $<0.005$ \\
& \multirow{1}{*}{balanced acc.} & $29.29$ & $<0.005$ & $28.09$ & $<0.005$  & $28.75$ & $<0.005$ \\
& \multirow{1}{*}{average F1} & $43.01$ & $<0.005$ & $42.09$ & $<0.005$  & $39.59$ & $<0.005$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{MLP}
& \multirow{1}{*}{accuracy} & $22.75$ & $<0.005$ & $20.43$ & $<0.005$  & $15.08$ & $<0.005$ \\
& \multirow{1}{*}{balanced acc.} & $28.00$ & $<0.005$ & $26.23$ & $<0.005$  & $23.61$ & $<0.005$ \\
& \multirow{1}{*}{average F1} & $39.31$ & $<0.005$ & $37.20$ & $<0.005$  & $33.22$ & $<0.005$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SAL}
& \multirow{1}{*}{accuracy} & $15.31$ & $<0.005$ & $13.35$ & $<0.005$  & $14.53$ & $<0.005$ \\
& \multirow{1}{*}{balanced acc.} & $22.10$ & $<0.005$ & $20.83$ & $<0.005$  & $20.34$ & $<0.005$ \\
& \multirow{1}{*}{average F1} & $31.36$ & $<0.005$ & $28.92$ & $<0.005$  & $31.16$ & $<0.005$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{pvalue_compare_to_baseline}
\end{table*}

==> preprint2020_Mobile Data/tables/stb_data_sources.tex <==
\begin{table}[h]
\begin{center}
%\small
%\fontsize{9}{10}\selectfont
\setlength{\tabcolsep}{7.5pt}
%\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|p{30mm}|p{45mm}|p{45mm}|}
\hline
Risk Domain &   Mobile Sensing Data   &   Example Features \\
\hline \hline
Emotional distress  &
Acoustic voice; Sentiment in communication (e.g., social media, text messaging); Facial expression (selfies); Music choice.  &
Fundamental frequency of voice; Positive or negative sentiment in language; Sad or anxious facial expression; Change in music selection.\\
\hline
Social dysfunction (e.g., thwarted belongingness, perceived burdensomeness) &
Self and social content in communication; Patterns of online communication (frequency, diversity of contacts); Geographic movement. &
Negative self-sentiment in language; Bullying or social rejection; Reduction in frequency and diversity of social contacts.\\
\hline
Sleep disturbance (biological diathesis)    &
Actigraphy; Light Sensor, Diurnal Patterns of phone Use.    &
Time in bed; Total sleep time; Sleep onset latency; Wake after sleep onset.\\
\hline
\end{tabular}
\end{center}
%\caption{}
\end{table}

==> tables/MLP_hyperparameters_apps.tex <==
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{MLP parameter configuration (Apps).}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l | c}
\Xhline{3\arrayrulewidth}
Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
hidden dim 1 & 128 \\
hidden dim 2 & 128, 64 \\
dropout rate & 0, 0.2, 0.5 \\
learning rate & 0.001 \\
batch size & 100 \\
epochs & 200 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{mlp_params_apps}
\end{table*}

==> tables/MLP_hyperparameters_bow.tex <==
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{MLP parameter configuration (Combined, BoW).}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l | c}
\Xhline{3\arrayrulewidth}
Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
hidden dim 1 & 1024, 512 \\
hidden dim 2 & 128, 64 \\
dropout rate & 0, 0.2, 0.5 \\
learning rate & 0.001 \\
batch size & 100 \\
epochs & 200 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{mlp_params_bow}
\end{table*}

==> tables/SAL_hyperparameters.tex <==
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{\names\ parameter configuration.}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l | c}
\Xhline{3\arrayrulewidth}
Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
$\lambda$ & 0.1, 1, 2, 3, 5, 10 \\
$\sigma$ & 1, 5, 10, 25, 50, 100 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{sal_params}
\end{table*}

==> tables/SVM_hyperparameters.tex <==
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{SVM parameter configuration. \\
*Integer kernel values denote the degree of a polynomial kernel.}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l | c }
\Xhline{3\arrayrulewidth}
Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
C & 0.1, 0.5, 1, 2, 3, 5, 10 \\
Kernel* & RBF, 2, 3, 5, 10 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{svm_params}
\end{table*}

==> tables/modalities_comparison.tex <==
\definecolor{gg}{RGB}{15,125,15}
\definecolor{rr}{RGB}{190,45,45}

\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\vspace{-4mm}
\centering
\caption{Comparison of mood prediction performance across different modalities. Best results in \textbf{bold}. For both accuracy and F1 score, models trained on both text and apps features outperform models trained using individual modalities. $\star$ and $\diamond$ denote that the difference between multimodal and unimodal (Text and Apps respectively) is statistically significant (p-value $<< 0.05$).}
\setlength\tabcolsep{5.0pt}
\begin{tabular}{l || c c c c | c c c c }
\Xhline{3\arrayrulewidth}
& \multicolumn{4}{c|}{{F1 score}} & \multicolumn{4}{c}{{Accuracy}} \\
Modalities & \textsc{Baseline} & \textsc{SVM} & \textsc{MLP} & \names &  \textsc{Baseline} & \textsc{SVM} & \textsc{MLP} & \names \\
\Xhline{0.5\arrayrulewidth}
Text + Apps &  $19.07$ & $\textbf{62.08}^{\diamond}$ & $\textbf{58.38}^{\star\diamond}$ & $\textbf{52.90}$ & $40.18$ & $\textbf{66.59}^{\diamond}$ & $\textbf{62.93}^{\star\diamond}$ & $\textbf{56.76}$ \\
Text & $19.07$ & $61.15 $ & $56.27$ & $52.63$ & $40.18$ & $65.83$ & $60.61$ & $56.08$ \\
Apps & $19.07$ & $58.65$ & $52.29$ & $51.32$ & $40.18$ & $62.65$ & $55.26$ & $55.68$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{modalities_comparison}
\end{table*}

==> tables/model_comparison.tex <==
\definecolor{gg}{RGB}{15,125,15}
\definecolor{rr}{RGB}{190,45,45}

\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{mood prediction}
\setlength\tabcolsep{5.0pt}
\begin{tabular}{l || c | c c c | c c c | c c c}
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{} & \multirow{2}{*}{Baseline} & \multicolumn{3}{c|}{{Text+Apps}} & \multicolumn{3}{c|}{{Text}} & \multicolumn{3}{c}{{Apps}} \\
& & \textsc{SVM} & \textsc{MLP} & \names & \textsc{SVM} & \textsc{MLP} & \names & \textsc{SVM} & \textsc{MLP} & \names \\
\Xhline{0.5\arrayrulewidth}
accuracy & $40.18$ & $66.59$ & $62.93$ & $55.49$ & $65.83$ & $60.61$ & $53.53$ & $62.65$ & $55.26$ & $54.20$ \\
average F1 & $19.07$ & $62.08$ & $58.38$ & $50.43$ & $61.15$ & $56.27$ & $47.98$ & $58.65$ & $52.29$ & $49.40$ \\
%balanced acc. & $33.33$ & $62.62$ & $61.34$ & $55.44$ & $61.43$ & $59.57$ & $54.16$ & $62.08$ & $56.95$ & $52.83$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{model_comparision}
\end{table*}

==> tables/privacy.tex <==
\definecolor{gg}{RGB}{15,125,15}
\definecolor{rr}{RGB}{190,45,45}

\begin{table*}[t!]
\vspace{-4mm}
\begin{minipage}{.45\linewidth}
\fontsize{9}{11}\selectfont
\caption{\textbf{Left:} We evaluate privacy in predicting user identity from representations learned by \textsc{MLP} and \names\ (\textbf{lower} accuracy is better), and find that \names\ effectively obfuscates user identity. \textbf{Right:} Tradeoff between performance (mood prediction F1 score, \textbf{higher} is better) and privacy (identity prediction accuracy, \textbf{lower} is better) \names\ provides a tunable parameter $\sigma$ which allows us to plot a range of (performance, privacy) points. Furthermore, using a multimodal model on text and app features pushes the Pareto front to obtain better performance and privacy at the same time.}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l || c c c }
\Xhline{3\arrayrulewidth}
& Text + Apps & Text & Apps \\
\Xhline{0.5\arrayrulewidth}
Raw features & $95.70$ & $92.65$ & $91.82$ \\ 
\textsc{MLP} & $79.04$ & $76.41$ & $85.94$ \\ 
\names & $\textbf{36.65}$ & $\textbf{38.38}$ & $\textbf{36.72}$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{privacy}
%
\end{minipage}
\hspace{4mm}
\vspace{-4mm}
\begin{minipage}{.55\linewidth}
\centering
\includegraphics[width=\textwidth]{images/tradeoff.png}
\end{minipage}

\vspace{-2mm}
\end{table*}

==> tables/pvalue_compare_modalities.tex <==
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{Comparing multimodal to single modalities}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l l || c c | c c }
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{} & \multirow{2}{*}{} & \multicolumn{2}{c|}{{Combined $\minus$ Text}} & \multicolumn{2}{c}{{Combined $\minus$ Apps}}  \\
& & $\Delta$ & p-value & $\Delta$ & p-value \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SVM}
& \multirow{1}{*}{accuracy} & $0.75$ & $0.2537$ & $3.93$ & $0.0038$ \\
& \multirow{1}{*}{balanced acc.} & $1.19$ & $0.1206$ & $0.54$ & $0.6768$ \\
& \multirow{1}{*}{average F1} & $0.92$ & $0.1664$ & $3.42$ & $0.0083$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{MLP}
& \multirow{1}{*}{accuracy} & $2.33$ & $0.0095$ & $7.67$ & $0.0025$ \\
& \multirow{1}{*}{balanced acc.} & $1.77$ & $0.0109$ & $4.39$ & $0.0035$ \\
& \multirow{1}{*}{average F1} & $2.11$ & $0.0183$ & $6.09$ & $0.0025$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SAL}
& \multirow{1}{*}{accuracy} & $1.96$ & $0.0463$ & $0.78$ & $0.3994$ \\
& \multirow{1}{*}{balanced acc.} & $1.28$ & $0.1931$ & $1.76$ & $0.2223$ \\
& \multirow{1}{*}{average F1} & $2.45$ & $0.234$ & $-0.10$ & $0.6006$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{pvalue_compare_modalities}
\end{table*}

\iffalse
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{p-value compared modalities (maybe include? really only MLP seems easy to talk about since it's clearly that Combined > BoW > App since they're all statistically significant. not really the case for svm though and def not for SAL)}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l l || c c | c c | c c }
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{} & \multirow{2}{*}{} & \multicolumn{2}{c|}{{Combined $\minus$ BoW}} & \multicolumn{2}{c|}{{Combined $\minus$ Apps}} & \multicolumn{2}{c}{{BoW $\minus$ Apps}} \\
& & $\Delta$ & p-value & $\Delta$ & p-value & $\Delta$ & p-value\\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SVM}
& \multirow{1}{*}{accuracy} & $0.75$ & $0.2537$ & $3.93$ & $0.0038$ & $3.18$ & $0.0183$ \\
& \multirow{1}{*}{balanced acc.} & $1.19$ & $0.1206$ & $0.54$ & $0.6768$ & $-0.65$ & $0.6394$ \\
& \multirow{1}{*}{average F1} & $0.92$ & $0.1664$ & $3.42$ & $0.0083$ & $2.50$ & $0.1013$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{MLP}
& \multirow{1}{*}{accuracy} & $2.33$ & $0.0095$ & $7.67$ & $0.0025$ & $5.35$ & $0.0063$ \\
& \multirow{1}{*}{balanced acc.} & $1.77$ & $0.0109$ & $4.39$ & $0.0035$ & $2.62$ & $0.0463$ \\
& \multirow{1}{*}{average F1} & $2.11$ & $0.0183$ & $6.09$ & $0.0025$ & $3.98$ & $0.0142$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SAL}
& \multirow{1}{*}{accuracy} & $1.96$ & $0.0463$ & $0.78$ & $0.3994$ & $-1.18$ & $0.7462$ \\
& \multirow{1}{*}{balanced acc.} & $1.28$ & $0.1931$ & $1.76$ & $0.2223$ & $0.49$ & $0.3994$ \\
& \multirow{1}{*}{average F1} & $2.45$ & $0.234$ & $-0.10$ & $0.6006$ & $-2.54$ & $0.9156$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{pvalue_compare_modalities}
\end{table*}
\fi

==> tables/pvalue_compare_to_baseline.tex <==

\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{p-value compared to baseline (seems pretty messy. don't want to include, will just say p-value is significant across all models, features, and metrics)}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l l || c c | c c | c c }
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{} & \multirow{2}{*}{} & \multicolumn{2}{c|}{{Combined}} & \multicolumn{2}{c|}{{Text}} & \multicolumn{2}{c}{{Apps}} \\
& & $\Delta$ & p-value & $\Delta$ & p-value & $\Delta$ & p-value\\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SVM}
 & \multirow{1}{*}{accuracy} & $26.41$ & $<0.005$ & $25.65$ & $<0.005$  & $22.47$ & $<0.005$ \\
& \multirow{1}{*}{balanced acc.} & $29.29$ & $<0.005$ & $28.09$ & $<0.005$  & $28.75$ & $<0.005$ \\
& \multirow{1}{*}{average F1} & $43.01$ & $<0.005$ & $42.09$ & $<0.005$  & $39.59$ & $<0.005$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{MLP}
& \multirow{1}{*}{accuracy} & $22.75$ & $<0.005$ & $20.43$ & $<0.005$  & $15.08$ & $<0.005$ \\
& \multirow{1}{*}{balanced acc.} & $28.00$ & $<0.005$ & $26.23$ & $<0.005$  & $23.61$ & $<0.005$ \\
& \multirow{1}{*}{average F1} & $39.31$ & $<0.005$ & $37.20$ & $<0.005$  & $33.22$ & $<0.005$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SAL}
& \multirow{1}{*}{accuracy} & $15.31$ & $<0.005$ & $13.35$ & $<0.005$  & $14.53$ & $<0.005$ \\
& \multirow{1}{*}{balanced acc.} & $22.10$ & $<0.005$ & $20.83$ & $<0.005$  & $20.34$ & $<0.005$ \\
& \multirow{1}{*}{average F1} & $31.36$ & $<0.005$ & $28.92$ & $<0.005$  & $31.16$ & $<0.005$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{pvalue_compare_to_baseline}
\end{table*}

==> tables/stb_data_sources.tex <==
\begin{table}[h]
\begin{center}
%\small
%\fontsize{9}{10}\selectfont
\setlength{\tabcolsep}{7.5pt}
%\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|p{30mm}|p{45mm}|p{45mm}|}
\hline
Risk Domain &   Mobile Sensing Data   &   Example Features \\
\hline \hline
Emotional distress  &
Acoustic voice; Sentiment in communication (e.g., social media, text messaging); Facial expression (selfies); Music choice.  &
Fundamental frequency of voice; Positive or negative sentiment in language; Sad or anxious facial expression; Change in music selection.\\
\hline
Social dysfunction (e.g., thwarted belongingness, perceived burdensomeness) &
Self and social content in communication; Patterns of online communication (frequency, diversity of contacts); Geographic movement. &
Negative self-sentiment in language; Bullying or social rejection; Reduction in frequency and diversity of social contacts.\\
\hline
Sleep disturbance (biological diathesis)    &
Actigraphy; Light Sensor, Diurnal Patterns of phone Use.    &
Time in bed; Total sleep time; Sleep onset latency; Wake after sleep onset.\\
\hline
\end{tabular}
\end{center}
%\caption{}
\end{table}
